Variable Elimination as Rewriting in a Linear Lambda Calculus

Variable Elimination (VE) is a classical exact inference algorithm for probabilistic graphical models such as Bayesian Networks, computing the marginal distribution of a subset of the random variables in the model. Our goal is to understand Variable Elimination as an algorithm acting on programs, here expressed in an idealized probabilistic functional language -- a linear simply-typed $\lambda$-calculus suffices for our purpose. Precisely, we express VE as a term rewriting process, which transforms a global definition of a variable into a local definition, by swapping and nesting let-in expressions. We exploit in an essential way linear types.

==> B-introduction.tex <==
%!TEX root = A-main.tex

\section{Introduction}

Probabilistic functional languages provide a general-purpose stochastic modelling language. 

in which several formalisms can be expressed. On the other side, specialised formalism, such as Bayesian Networks, come with efficient inference algorithms --- in particular  \emph{exact inference} algorithms, the simplest one being Variable Elimination (\VE{} for short) --- which are lost when moving to programs. Here, we provide an inference algorithm which essentially mimic \VE{} in an idealised probabilistic functional language --- a linear simply-typed $\lambda$-calculus. When we run our algorithm on a stochastic program representing a Bayesian network, its computational behaviour is the same as that of standard \VE{} for Bayesian networks, and the cost is of the same complexity order. Let us explain the main ideas in more details. 

Bayesian networks describe a set of random variables by their conditional dependences. Let us restrict ourself to boolean random variables, \ie variables $x$ representing a boolean value $\True$ or $\False$ with some probability.\footnote{The results of this paper trivially extends to the case of random variables over countable sets of outcomes, while a more sophisticated framework is necessary in case of continuous random variables.} Such a variable can be described as a vector of two non-negative real numbers $x = (\ScalA_\True, \ScalA_\False)$ quantifying the probability $\ScalA_\True$ (resp.~$\ScalA_\False$) of sampling $\True$ (resp.~$\False$) from $x$.% \ie{} $\ScalA_\True+\ScalA_\False=1$.

\begin{wrapfigure}{L}{0.37\textwidth}
%inside [] number of text rows
%\vspace{-10pt}
\centering
	\tikz{
		\node [circle, draw] (1) at (0, 0.75) {$x_1$};
		\node [circle, draw] (2) at (1, 0) {$x_2$};
		\node [circle, draw] (3) at (2.5, 0) {$x_3$};	
		\node [circle, draw] (4) at (3.5, 0.75) {$x_4$};		
		\node [circle, draw] (5) at (2.5, 1.5) {$x_5$};	
		\node [circle, draw] (6) at (1, 1.5) {$x_6$};	
		
		\graph[edges={thick}]  { 
			(1) -> (2) -> (3) -> (5) -> (6) ;
			(2) -> (6) ;
			(4) -> (5) ;
		};
	}
% eliminate x1, x2, x4, x5
%\vspace{-10pt}
\caption{A Bayesian network.}\label{fig:bayesian_graph}
%\vspace{-10pt}
\end{wrapfigure}
Figure~\ref{fig:bayesian_graph} depicts an example of Bayesian network. It is a directed acyclic graph $\mathcal G$ where nodes are associated with random variables and the arrows describe conditional dependences between these variables. For instance, in Figure~\ref{fig:bayesian_graph} the variable $x_5$ depends on the values sampled from $x_3$ and $x_4$, and, in its turn, it affects the probability of which boolean we can sample from $x_6$. The network does not give a direct access to a vector $(\ScalA_\True, \ScalA_\False)$ describing $x_5$ by its own, but only to a stochastic matrix $\StocA_5$ quantifying 
the conditional dependence of $x_5$ with respect to $x_3$ and $x_4$. Formally, $\StocA_5$ is a matrix with 
four lines, representing the four possible outcomes of a joint sample of $x_3$ and $x_4$ (\ie $(\True, \True)$,  $(\True, \False)$, $(\False, \True)$, $(\False, \False)$), and two columns, representing the two possible outcomes of $x_5$. The matrix is \emph{stochastic} in the sense that each line represents a probabilistic distribution of booleans: for instance, $(\StocA_5)_{(\True, \False), \True}=0.4$ and $(\StocA_5)_{(\True, \False), \False}=0.6$ mean that $\True$ can be sampled from $x_5$  with 40\% of chances, while $\False$ with 60\%, whenever $x_3$ has been observed to be $\True$ and $x_4$ to be $\False$. 

Having such a graph $\mathcal G$ and the stochastic matrices $\StocA_1$, $\StocA_2$, $\StocA_3$, \etc associated with its nodes, a typical question is to compute the joint probability of a subset of the variables of  $\mathcal G$. For example, the vector $(x_3, x_6)$ giving the probability of the possible outcomes of $x_3$ and $x_6$. One can do that by first computing the joint distributions of all variables in the graph in a shot and then summing out the ones we are not interest in. This will give, for every possible boolean value $b_3,b_6\in\{\True,\False\}$ taken by, respectively, $x_3$ and $x_6$, the following expression:
\begin{equation}
\label{eq:let_term_semantics1}
	\sum_{
		\substack{
			b_1,b_2,b_4,
			b_5\in \{\True, \False\}
		}
	}
	(\StocA_1)_{b_1}
	(\StocA_2)_{b_1, b_2}
	(\StocA_3)_{b_2, b_3}
	(\StocA_4)_{b_4}
	(\StocA_5)_{(b_3, b_4), b_5}
	(\StocA_6)_{(b_2, b_5), b_6}\,.
\end{equation}
For each of  the $2^2$ possible values of the indexes $(b_3, b_6)$ we have a sum of $2^4$ terms, \ie we have an order of $2^6$ basic operations to compute the joint probability of $(x_3, x_6)$. This method is unfeasible in general as it requires a number of operations exponential in the size of $\mathcal G$. Luckily, one can take advantage of the conditional dependences underlined by $\mathcal G$ to get a better factorisation of~\eqref{eq:let_term_semantics1}. For example:
\begin{equation}
\label{eq:let_term_semantics2}
	\sum_{b_5}\!
		\left(\!\sum_{b_2}\!
		\left(\!\sum_{b_1}
			(\StocA_1)_{b_1}
			(\StocA_2)_{b_1, b_2}
		\!\right)
		(\StocA_3)_{b_2, b_3}
		(\StocA_6)_{(b_2, b_5), b_6}
		\!\right)\!
		\left(\!
		\sum_{b_4}
		(\StocA_4)_{b_4}
		(\StocA_5)_{(b_3, b_4), b_5}
		\!\right)\!.
\end{equation}
Let us denote by $\FactA^i$ the intermediate factor in \eqref{eq:let_term_semantics2} identified by the sum over $b_i$: for example $\FactA^2$ is the sum $\sum_{b_2}\FactA^1_{b_2}(\StocA_3)_{b_2, b_3}(\StocA_6)_{(b_2, b_5), b_6}$. Notice that if we suppose to have memorised the results of the computation of $\FactA^1$, the cost of computing $\FactA^2$ is of order of $2^4$, i.e.~exponential in the number of different indexes $b_j$'s appearing in the expression defining $\FactA^2$. By applying this reasoning to all factors in~\eqref{eq:let_term_semantics2}, one can notice that the whole computation requires an order of $2^4$ basic operations: we have gained a factor of $2^2$ with respect to \eqref{eq:let_term_semantics1}.
%
%
%\begin{align*}
%%observe x3, x6
%%elimin x1
%\FactA^1_{a_2}&=\sum_{a_1}
%	(\StocA_1)_{a_1}
%	(\StocA_2)_{a_1, a_2}\,,
%&
%%elimin x2
%\FactA^2_{a_3, a_5, a_6}&=\sum_{a_2}
%	\FactA_{a_2}
%	(\StocA_3)_{a_2, a_3}
%	(\StocA_6)_{(a_2, a_5), a_6}\,,
%\\
%%elmin x4
%\FactA^4_{a_5}&=\sum_{a_4}
%	(\StocA_4)_{a_4}
%	(\StocA_5)_{a_4, a_5}\,,
%&
%%elimin x5
%\ScalA_{a_3, a_6}&=\sum_{a_5}
%	\FactA^4_{a_5}
%	\FactA^2_{a_3, a_5, a_6}\,.
%\end{align*}
%%
%%\begin{equation}
%%\label{eq:let_term_semantics2}
%%	\ScalA_{b_5, b_6}=
%%	\sum_{a_3,a_4,a_5}
%%	\sum_{a_1}
%%		\sum_{a_2}
%%		(\StocA_3)_{a_2, a_3}
%%		(\StocA_4)_{a_2, a_4}	
%%		(\StocA_6)_{(a_2, a_5), b_6}
%%	(\StocA_5)_{a_4, b_5}
%%\end{equation}
%

The variable elimination algorithm is one among the simplest algorithm in Bayesian inference performing factorisations like \eqref{eq:let_term_semantics2} in order to compute joint distributions. The name is motivated by the fact that a factorisation is characterised by an ordered sequence of unobserved (or marginalised) variables to eliminate, \ie to sum out. The factorisation in \eqref{eq:let_term_semantics2} is induced by the sequence $(x_1,x_2,x_4,x_5)$:  $\FactA^1$ eliminates variable $x_1$, 
$\FactA^2$ then eliminates variable $x_2$, and so on. Different orders yield to different factorisations with different performances, \eg{} the inverse order $(x_5,x_4,x_2,x_1)$ is as inefficient as \eqref{eq:let_term_semantics1}. 

In the literature, these factorisations are usually described as collections of factors, basically vectors, and the \VE{} algorithm is presented as an iterative algorithm acting on such collections. In this paper we propose a framework that gives more \emph{structure} to this picture, expressing \VE{} as a program transformation, building a factorisation by the induction on the structure of a program. More precisely, our main contributions are:
\begin{enumerate}
\item we identify a fragment $\LetCalculus$ of the linear simply-typed $\lambda$-calculus able to represent \emph{any} factorisation of a Bayesian network query as a $\lambda$-term;
\item we express the \VE{} algorithm as a rewriting over the $\lambda$-terms in $\LetCalculus$, which reduces the scope of the marginalised variables. 
\end{enumerate}
While the idea behind VE is simple, crafting  an algorithm  on terms which is able to 
implement any elimination order is a non-trivial contribution --- we rely  a fine understanding 
coming from linear logic \cite{ll}. In pioneering work 
  on probabilistic programming languages \cite{KollerMP97}, the authors define a general purpose  functional language with the ability  to model Bayesian networks, and  provide  an algorithm which mimics variable elimination. The limit  is however that the algorithm there can only implement a specific elimination ordering (the one determined  by the lazy evaluation  implicit in the algorithm), which   might not be  the  most efficient. Our approach allows to implement \emph{any} elimination ordering. 
%
%\todoc{Maybe we just state an objective fact like this,  without explicitely stating that we solve the problem left open in \cite{KollerMP97}?} 
%



\begin{wrapfigure}{R}{0.38\textwidth}
%\vspace{-20pt}
\begin{minipage}{0.38\textwidth}
\[
	\begin{array}{l}
	\mathtt{let }\, x_1 = \StocA_1\, \mathtt{ in}\\
	\mathtt{let }\, x_2 = \StocA_2 x_1\, \mathtt{ in}\\
	\mathtt{let }\, x_3 = \StocA_3 x_2\, \mathtt{ in}\\
	\mathtt{let }\, x_4 = \StocA_4 \, \mathtt{ in}\\
	\mathtt{let }\, x_5 = \StocA_5 (x_3, x_4)\, \mathtt{ in}\\
	\mathtt{let }\, x_6 = \StocA_6 (x_2, x_5)\, \mathtt{ in}\\
	(x_3, x_6)
	\end{array}
\]
\end{minipage}
%\vspace{-10pt}
\caption{A let-term $\LetTerm$.}\label{fig:let-term}
%\vspace{-10pt}
\end{wrapfigure}
The reader can easily convince herself that the query about the joint distribution $(x_3, x_6)$ to the Bayesian network in Figure~\ref{fig:bayesian_graph} can be expressed by the let-term $\LetTerm$ in Figure~\ref{fig:let-term}, where we have enriched the syntax with the constants representing the stochastic matrices. We suppose $\Let xe{e'}$ as a syntactic sugar for $(\lambda x. e')e$, so the term $\LetTerm$ can be seen as a $\lambda$-term, which is moreover typable in a linear type system like the one in Figure~\ref{fig:terms_types}. The fact that some variables $x_i$ have more free occurrences in sub-terms of $\LetTerm$ is not in contrast with the linearity feature of the term, as let-expressions are supposed to be evaluated following a call-by-value strategy, and ground values (as for example booleans) can be duplicated in linear systems (see Remark~\ref{rk:typing_as_MLL} for more details).

Terms of this type are associated in quantitative semantics such as \cite{danosehrhard,LairdMMP13} with factorisations giving the joint distribution of the output variables. In particular, the interpretation of $\LetTerm$ gives a factorisation which is as inefficient as~\eqref{eq:let_term_semantics1} in computing the joint distribution of $\Seq{x_3,x_6}$ (Example~\ref{ex:semantics_let}). 


%\begin{wrapfigure}{R}{0.38\textwidth}
%%\vspace{-20pt}
%\begin{minipage}{0.38\textwidth}
%\[
%	\begin{array}{l}
%	\mathtt{let }\, x_3, f =\\ 
%	\qquad\mathtt{let }\, x_2 =\\
%	\qquad\qquad\mathtt{let }\, x_1 = \StocA_1\, \mathtt{ in}\\	
%	\qquad\qquad\StocA_2 x_1\,\mathtt{ in}\\
%	\qquad(\StocA_3 x_2, \lambda x_5.\StocA_6 (x_2, x_5))\,\mathtt{ in}\\
%	\mathtt{let }\, x_5 =\\
%	\qquad\mathtt{let }\, x_4 = \StocA_4 \, \mathtt{ in}\\
%	\qquad\StocA_5 (x_3, x_4)\, \mathtt{ in}\\
%	(x_3, f x_5)
%	\end{array}
%\]
%\end{minipage}
%%\vspace{-10pt}
%\caption{A let-term for factorisation \eqref{eq:let_term_semantics2}.}\label{fig:let-term}
%%\vspace{-10pt}
%\end{wrapfigure}
In fact, $\LetCalculus$ is sufficiently expressive to represent all possible factorisations of~\eqref{eq:let_term_semantics1}, \eg \eqref{eq:let_term_semantics2}. The main idea for such a representation arises from the observation that summing-out variables in the semantics corresponds in the syntax to make a let-in definition local to a sub-expression. For example, the factor $\FactA^1 = \sum_{b_1}(\StocA_1)_{b_1}(\StocA_2)_{b_1, b_2}$ of \eqref{eq:let_term_semantics2} can be easily obtained by making the variable $x_1$ local to the definition of $x_2$, creating a $\lambda$-term $e^1$ of the shape $\Let{x_1}{\StocA_1}{\StocA_2 x_1}$ and replacing the first two definitions of $\LetTerm$ with $\Let{x_2}{e^1}{\dots}$. In fact, the denotation of $e^1$ is exactly $\FactA^1$. What about $\FactA^2$? Here the situation is subtler as in order to make local the definition of $x_2$ one should gather together the definitions of  $x_3$ and $x_6$, but the definition of $x_6$ depends on a variable $x_5$ which in its turn depend on $x_3$, so a simple factor of ground types (\ie tensors of booleans) will generate a dependence cycle. Luckily, we can use a (linear) functional type, defining a $\lambda$-term $e^2$ as $\Let{x_2}{e^1}{\Seq{\StocA_3 x_2, \lambda x_5.\StocA_6 \Seq{x_2, x_5}}}$ and then transforming $\LetTerm$ into: $\Let{(x_3, f)}{e^2}{\dots\Let{x_6}{f x_5}{\Seq{x_3,x_6}}}$. Again, we can notice that the denotation of $e^2$ is exactly $\FactA^2$. Figure~\ref{fig:example_reduction} details\footnote{Actually, the expressions $e^1$ and $e^2$ in Figure~\ref{fig:example_reduction}  are a bit more cumbersome that the ones here discussed because of some bureaucratic let-in produced by a more formal treatment. This difference is however inessential and can be avoided by adding some optimising post-processing.} the whole rewriting mimicking the elimination of the variables $(x_1, x_2, x_4, x_5)$ applied to $\LetTerm$.  This paper shows how to generalise this reasoning to any let-term.

\paragraph{Contents of the paper.} Section~\ref{sect:syntax} defines the linear $\lambda$-calculus $\LetCalculus$. In particular, Figure~\ref{fig:terms_types} gives the linear typing system, which is a fragment of multiplicative linear logic \cite{ll} (Remark~\ref{rk:typing_as_MLL}). Figure~\ref{fig:denotation_terms} sketches the quantitative semantics of $\LetCalculus$ as weighted relations \cite{LairdMMP13}. By using an enrichment of this latter, a variant of probabilistic coherence spaces \cite{danosehrhard}, we achieve a nice property of the terms of $\LetCalculus$, namely that the total mass of their denotation is easily computable from the type of the terms (Proposition~\ref{prop:totality-mass}). Section~\ref{sect:factors} formalises the notion of factorisation as a set of factors (Definition~\ref{def:factor}) and show how to associate a factorisation with a specific class of terms in $\LetCalculus$, called \emph{let-terms} (Definition~\ref{def:factor_of_let_term}). Definition~\ref{def:VE_factors} then recalls the standard \VE{} algorithm as acting on sets of factors, denoted here by $\VEF$. The core of our contribution is Section~\ref{sect.VE_as_let_rewriting}, capturing \VE{} as a let-term transformation (Definition~\ref{def:VE}), denoted here by $\VEL$, using the rewriting rules of Figure~\ref{fig:let-rewriting}. We prove the correspondence between the two versions of $\VE$ in Theorem~\ref{th:soundnessVE_Let} and Corollary~\ref{cor:soundnessVE_Let_nary}, stating the $\VEL$ soundness and completeness with respect to $\VEF$. 

\paragraph{Related work.}
%Let us adopt \cite{Darwiche2009} as a general reference on Bayesian networks, although this notion dates back to \cite{Pearl88}  and the variable elimination algorithm at least to \cite{ZhangP94}\todom{sure of this reference?}.
%	\todoc{\textbf{Per ZhangP95: }Versioni di algoritmi che usano la stessa idea di fattorizzazione (come sum-product o message passing) sono piu' anziane.  Ma \cite{ZhangP94} e' la prima formulazione dell'algoritmo semplice che seguiamo qui, quello che Koller e Darwiche chiamano Variable Elimination}. 
We adopt \cite{Darwiche2009} as a general reference on Bayesian networks \cite{Pearl88}. Variants of factorisation algorithms were invented independently in multiple communities. The algorithm of variable elimination which we consider here was first formalised in \cite{ZhangP94}. The relationship between Bayesian networks and program semantics has been put forward in the setting of string diagrams, \eg \cite{ChoJ19,JacobsKZ19},~and the denotational foundations of probabilistic programming, \eg \cite{Stein2021CompositionalSF,Paquet21}. %\textcolor{blue}{
However, these approaches do not take into consideration the computational efficiency, which is the very reason motivating Bayesian networks, and inference algorithms such as variable elimination.
%}
 %\textcolor{red}{[and formalised as a program transformation]}.
%  Let us underline that $\LetCalculus$  identifies a fragment of multiplicative linear logic~\cite{ll} extended with stochastic matrices, so it can be modeled by $\star$-autonomous categories like \cite{danosehrhard} without the need of being compact closed\todoc{Questa frase e' un po' sconnessa dal resto del related work. Non mi e' chiaro cosa  si vuole dire}.
 We formalise the \VE{} algorithm as a program transformation over $\lambda$-terms.  Several heuristics are available in the literature to compute an efficient elimination order, we refer the reader to \cite{Darwiche2009}.
 
  %We focus on a theoretical framework, giving a proof of soundness and completeness (Theorem~\ref{th:soundnessVE_Let}, Corollary~\ref{cor:soundnessVE_Let_nary}). %An implementation of this framework will be discussed in future work. 
 
 %\todoc[inline]{It seems delicate to say that ``\textit{in our knowledge, this is the first time that a basic inference algorithm like the variable elimination algorithm is \textcolor{red}{and formalised as a program transformation}}''.}

%\todom[inline]{cite \cite{KollerMP97} fa variable elimination su termini  (dicendo che sono in grado di eliminare rispetto a certi ordini, non necessariamente ottimali)}
 %
% Taken from the paper: It can be shown that, applied to a Bayesian network, our algorithm mimics the standard vari- able elimination algorithm, using the elimination ordering implied by the lazy evaluation behavior of the algorithm. Unfortunately, this elimination algorithm might not be the optimal ordering for a given Bayesian network.
%



%%%%%%%%


